Mediation of Collisionless Turbulent Dissipation Through Cyclotron Resonance

The dissipation of magnetized turbulence is fundamental to understanding energy transfer and heating in astrophysical systems. Collisionless interactions, such as resonant wave-particle process, are known to play a role in shaping turbulent astrophysical environments. Here, we present evidence for the mediation of turbulent dissipation in the solar wind by ion-cyclotron waves. Our results show that ion-cyclotron waves interact strongly with magnetized turbulence, indicating that they serve as a major pathway for the dissipation of large-scale electromagnetic fluctuations. We further show that the presence of cyclotron waves significantly weakens observed signatures of intermittency in sub-ion-kinetic turbulence, which are known to be another pathway for dissipation. These observations results suggest that in the absence of cyclotron resonant waves, non-Gaussian, coherent structures are able to form at sub-ion-kinetic scales, and are likely responsible for turbulent heating. We further find that the cross helicity, i.e. the level of Alfv\'enicity of the fluctuations, correlates strongly with the presence of ion-scale waves, demonstrating that dissipation of collisionless plasma turbulence is not a universal process, but that the pathways to heating and dissipation at small scales are controlled by the properties of the large-scale turbulent fluctuations. We argue that these observations support the existence of a helicity barrier, in which highly Alfv\'enic, imbalanced, turbulence is prevented from cascading to sub-ion scales thus resulting in significant ion-cyclotron resonant heating. Our results may serve as a significant step in constraining the nature of turbulent heating in a wide variety of astrophysical systems.

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


